Exploiting Data Longevity for Enhancing the Lifetime of Flash-based Storage Class Memory

Storage-class memory (SCM) combines the benefits of a solid-state memory, such as high-performance and robustness, with the archival capabilities and low cost of conventional hard-disk magnetic storage. Among candidate solid-state nonvolatile memory technologies that could potentially be used to construct SCM, flash memory is a well-established technology and have been widely used in commercially available SCM incarnations. Flash-based SCM enables much better tradeoffs between performance, space and power than disk-based systems. However, write endurance is a significant challenge for a flash-based SCM (each act of writing a bit may slightly damage a cell, so one flash cell can be written 10^4--10^5 times, depending on the flash technology, before it becomes unusable). This is a well-documented problem and has received a lot of attention by manufactures that are using some combination of write reduction and wear-leveling techniques for achieving longer lifetime. In an effort to improve flash lifetime, first, by quantifying data longevity in an SCM, we show that a majority of the data stored in a solid-state SCM do not require long retention times provided by flash memory (i.e., up to 10 years in modern devices); second, by exploiting retention time relaxation, we propose a novel mechanism, called Dense-SLC (D-SLC), which enables us perform multiple writes into a cell during each erase cycle for lifetime extension; and finally, we discuss the required changes in the flash management software (FTL) in order to use this characteristic for extending the lifetime of the solid-state part of an SCM. Using an extensive simulation-based analysis of a flash-based SCM, we demonstrate that D-SLC is able to significantly improve device lifetime (between 5.1X and 8.6X) with no performance overhead and also very small changes at the FTL software.

==> eval-sense.tex <==
\section{Sensitivity Analysis}




\subsection{Different Voltage Drift Distances}
\label{sec:sense-drift}



\subsubsection{Non-Uniform Device Characteristics}

The voltage drift distance as a function of the retention time and the P/E cycles (discussed in Section \ref{drift}) can be a little longer or shorter, depending on the device characteristics. Specifically, it is affected by a wide variety of device design factors (such as vendors, technology nodes, material-level characteristics), which makes a need to evaluate our scheme in different devices exhibiting varying drift patterns. Hence, in addition to the configuration evaluated in Section \ref{sec:eval-base}, we employ two more devices by changing the scaling constant (K) of Equation \ref{eq:drift-model}. The three evaluated systems in this experiment are as follows:


\begin{itemize}[leftmargin=*]
	\item \textbf{Weak}: In this device, the voltage state drifts longer under the same P/E cycles and retention times. K is set to $5 \times 10^{-4}$.  
	\item \textbf{Normal}: It is the configuration employed so far (Section \ref{sec:eval-base}). The scaling constant K is set to $4 \times 10^{-4}$.   
	\item \textbf{Strong}: The voltage state in this device drifts shorter under the same P/E cycles and retention times (K is set to $3 \times 10^{-4}$).   
\end{itemize}


The three devices have different mappings of state modes to their blocks for each pair of P/E cycles and retention times, which are listed in Table \ref{tab:mode-assign-3-sense-drift}. For example, \emph{Strong} device can store data whose retention times are between 1 and 10 hours in blocks with 8-state mode at any time (P/E cycle), whereas in \emph{Weak} device, such data should be placed only in blocks with 4-state mode after 10K P/Es.


\begin{table}[!h]
\caption{Block state mode assignment (2, 4, or 8-state mode) for different I/O retention times as a function of the block age in Weak / Normal / Strong devices.}
\label{tab:mode-assign-3-sense-drift}
%\small
\footnotesize
%\vspace
\begin{tabular}{|p{0.8in}||c|c|c|c|c|  }
\hline 
\textbf{Retention}		& \multicolumn{5}{|c|}{\textbf{Number of Erases to the Block} } \\ \cline{2-6}
\textbf{Time}	&	0$\sim$10K 	&	10$\sim$20K	&	20$\sim$30K	&	30$\sim$40K	&	40$\sim$50K	 \\ 
\hline\hline 
$\le$1 Hour			&	8/8/8	& 	8/8/8	&	8/8/8	&	8/8/8	&	8/8/8	\\
\hline 
1 $\sim$10 Hours		&	8/8/8	&   	4/8/8	&	4/8/8	&	4/4/8	&	4/4/8	\\
\hline 
10 Hours $\sim$ 3 Days	& 	4/4/8	&	4/4/4	&	2/4/4	&	2/2/4	&	2/2/4	\\
\hline 
$\ge$ 3 Days 		& 	2/2/2	&	2/2/2	&	2/2/2	&	2/2/2	&	2/2/2	\\
\hline
\end{tabular}
%\vspace{-5pt}
\end{table}

\begin{figure*}[t]
\centering
%\vspace{-5pt}
\includegraphics[width=0.98\linewidth, bb= 0 0 3312 720]{graphs/sense-drift-life.eps}
%\vspace{-8pt}
\caption{Lifetime improvement brought by our scheme in Weak, Normal, and Strong devices, normalized to the baseline SLC.}
\label{fig:sense-drift-life}
%\vspace{-6pt}
\end{figure*}



\begin{figure*}
\centering
	\begin{subfigure}{.28\linewidth}
		\centering
		\includegraphics[width=0.99\linewidth]{graphs/pwe-web_1-weak.eps}
		\caption{web\textunderscore1 in Weak}\label{fig:pwe-sense-drift-web_1-weak}
	\end{subfigure}
	\begin{subfigure}{.28\linewidth}
		\centering
		\includegraphics[width=0.99\linewidth]{graphs/pwe-web_1.eps}
		\caption{web\textunderscore1 in Normal}\label{fig:pwe-sense-drift-web_1-normal}
	\end{subfigure}
	\begin{subfigure}{.28\linewidth}
		\centering
		\includegraphics[width=0.99\linewidth]{graphs/pwe-web_1-strong.eps}
		\caption{web\textunderscore1 in Strong}\label{fig:pwe-sense-drift-web_1-strong}
	\end{subfigure}
\caption{Percentages of blocks with 2, 4, and 8 states, when running \emph{web\textunderscore1} on Weak, Normal, and Strong devices.}
\label{fig:pwe-sense-drift-web_1}
\end{figure*}




\begin{figure*}
\centering
	\begin{subfigure}{.28\linewidth}
		\centering
		\includegraphics[width=0.99\linewidth]{graphs/pwe-prn_0-weak.eps}
		\caption{prn\textunderscore0 in Weak}\label{fig:pwe-sense-drift-prn_0-weak}
	\end{subfigure}
	\begin{subfigure}{.28\linewidth}
		\centering
		\includegraphics[width=0.99\linewidth]{graphs/pwe-prn_0.eps}
		\caption{prn\textunderscore0 in Normal}\label{fig:pwe-sense-drift-prn_0-normal}
	\end{subfigure}
	\begin{subfigure}{.28\linewidth}
		\centering
		\includegraphics[width=0.99\linewidth]{graphs/pwe-prn_0-strong.eps}
		\caption{prn\textunderscore0 in Strong}\label{fig:pwe-sense-drift-prn_0-strong}
	\end{subfigure}
\caption{Percentages of blocks with 2, 4, and 8 states, when running \emph{prn\textunderscore0} on Weak, Normal, and Strong devices.}
\label{fig:pwe-sense-drift-prn_0}
%\vspace{-6pt}
\end{figure*}



\subsubsection{Effectiveness of Our Schemes under Different Devices.}

Figure \ref{fig:sense-drift-life} compares the lifetime improvements achieved by our scheme in three different devices. \emph{In general, one can observe that our scheme brings more lifetime improvements in stronger devices (where their voltage drifts are shorter) than in weaker devices (whose voltage drifts are longer)}. These results come from two major reasons:


\begin{itemize}[leftmargin=*]
	\item In all devices, the inter-update times (retention times) of data remain unchanged. Note that this is an attribute of workloads, regardless of device characteristics.
	\item In stronger devices, more and more data with the same retention times can be stored in blocks with more states. For example, according to Table \ref{tab:mode-assign-3-sense-drift}, the Strong device allows data whose retention times are between 10 hours and 3 days to be stored in blocks with 0 to 10K P/Es as 8-state modes, while such data should be accommodated in 4-state mode blocks until 10K P/Es in the Normal or Weak devices.
\end{itemize}


%in Figure \ref{fig:pwe-sense-drift}

The PWE analysis shows how our scheme increases PWE values as the target device becomes drift-resistant (i.e., stronger). As a representative, Figures \ref{fig:pwe-sense-drift-web_1-weak}, \ref{fig:pwe-sense-drift-web_1-normal}, and \ref{fig:pwe-sense-drift-web_1-strong} show the percentage of blocks with 2, 4, and 8 states, when running \emph{web\textunderscore1} in Weak, Normal, and Strong devices, respectively. (Note that the PWE analysis for all other workloads can be referred in Appendix). One can see from these figures that the ratios of blocks with 4 states (black area) and with 2 states (red area) gradually decrease, as the drift resistance increases from Weak to Strong devices. Specifically, the Weak device needs blocks with 2 states to store data whose retention times range from 10 hours to 3 days from around 1,000K hours (i.e., 20K P/Es), whereas such data require 2-state mode blocks after around 1,500K hours (i.e., 30K P/Es) in the Normal device. On the other hand, no 2-state mode block is needed to store such data in Strong device; no red cliff is observed in Figure \ref{fig:pwe-sense-drift-web_1-strong}.


One might also observe that, in some workloads such as \emph{prn\textunderscore0} and \emph{proj\textunderscore0}, the lifetime improvements stay quite low in the Weak device. This phenomenon of these workloads can be explained by the PWE analysis. Figures \ref{fig:pwe-sense-drift-prn_0-weak}, \ref{fig:pwe-sense-drift-prn_0-normal}, and \ref{fig:pwe-sense-drift-prn_0-strong} show the percentage of blocks with three different states when executing \emph{prn\textunderscore0}, a representative of such workloads, in the Weak, Normal, and Strong devices, respectively. The ratio of blocks with 4 states is very low in the Normal device, and it is almost removed in the Strong device. In contrast, the percentage of 4-state mode blocks largely increases in the Weak device; the black area in Figure \ref{fig:pwe-sense-drift-prn_0-weak} appears remarkably. It is because the data whose retention times range 1 to 10 hours need 4-state mode blocks so early (i.e., after 10K P/Es), while such data need them after 30K P/Es in the Normal device and none of them throughout the lifespan in the Strong device.

%reveals that the ratio of blocks with less states (i.e., 2 or 4 states) largely increases in the Weak device

\begin{table}
\caption{The assignment of state modes (2, 4, 5, 6, or 8-state mode) to blocks in our schemes supporting 2/3/4/5 modes.}
\label{tab:mode-assign-5-sense-mode}
%\small
\footnotesize
%\vspace
\begin{tabular}{|p{0.8in}||c|c|c|c|c|  }
\hline 
\textbf{Retention}		& \multicolumn{5}{|c|}{\textbf{Number of Erases to the Block} } \\ \cline{2-6}
\textbf{Time}	&	0$\sim$10K 	&	10$\sim$20K	&	20$\sim$30K	&	30$\sim$40K	&	40$\sim$50K	 \\ 
\hline\hline 
$\le$1 Hour			&	8/8/8/8 &	8/8/8/8 &	8/8/8/8 &	8/8/8/8 &	8/8/8/8 \\
\hline 
1 $\sim$10 Hours		&	8/8/8/8 &	8/8/8/8 &	8/8/8/8 &	\textbf{2/4/5/6} & \textbf{2/4/5/6} \\
\hline 
10 Hours$\sim$3 Days	&  \textbf{2/4/5/6} & \textbf{2/4/5/5} & \textbf{2/4/4/4} & 2/2/2/2 & 2/2/2/2 \\
\hline 
$\ge$ 3 Days 			& 	2/2/2/2 &	2/2/2/2 &	2/2/2/2 &	2/2/2/2 &	2/2/2/2 \\
\hline
\end{tabular}
%\vspace{-5pt}
\end{table}


\subsection{Different Numbers of State Modes}


\subsubsection{Varying Granularities of Our Scheme}

So far, our scheme employs ``three'' different modes, which are 2, 4, and 8-state modes. However, one might want to manage voltage drifts in finer granularities by employing additional modes such as 5 and 6-state modes. Thus, we evaluate our scheme supporting different numbers of state modes; we compare the following four systems:

\begin{itemize}[leftmargin=*]
	\item \textbf{2-Mode}: It adds one additional mode (8-state) to the baseline SLC; so, this system has two modes (2 and 8-state modes).
	\item \textbf{3-Mode}: This system is what we considered throughout the paper, which has three state modes (2, 4, and 8-state modes).
	\item \textbf{4-Mode}: One more state mode is added to the Mode-3, which has four state modes (2, 4, 5, and 8-state modes).
	\item \textbf{5-Mode}: Managing voltage drift more precisely, it supports five different modes (2, 4, 5, 6, and 8-state modes).
\end{itemize}


Increasing the number of supporting modes changes the mapping of their state modes to blocks. Table \ref{tab:mode-assign-5-sense-mode} provides the different mappings of state modes to their blocks for each pair of P/E cycles and retention times in the four evaluated systems. 



\begin{figure}
\centering
%\vspace{-5pt}
\begin{subfigure}{.49\linewidth}
	\centering
	\includegraphics[width=0.99\linewidth, bb= 0 0 648 504]{graphs/sense-mode-life-same.eps}
	\caption{Low-beneficial workloads}\label{fig:sense-mode-life-same}
\end{subfigure}
\begin{subfigure}{.49\linewidth}
	\centering
	\includegraphics[width=0.99\linewidth, bb= 0 0 648 504]{graphs/sense-mode-life-increase.eps}
	\caption{High-beneficial workloads}\label{fig:sense-mode-life-increase}
\end{subfigure}
%\vspace{-8pt}
\caption{Lifetime improvement brought by device under varying numbers of states, normalized to the baseline SLC.}
\label{fig:sense-mode-life}
%\vspace{-6pt}
\end{figure}




\begin{figure*}
\centering
	\begin{subfigure}{.24\linewidth}
		\centering
		\includegraphics[width=0.99\linewidth]{graphs/pwe-src1_2-m2.eps}
		\caption{src1\textunderscore2 in 2-Mode}\label{fig:pwe-sense-mode-src1_2-m2}
	\end{subfigure}
	\begin{subfigure}{.24\linewidth}
		\centering
		\includegraphics[width=0.99\linewidth]{graphs/pwe-src1_2.eps}
		\caption{src1\textunderscore2 in 3-Mode}\label{fig:pwe-sense-mode-src1_2-m3}
	\end{subfigure}
	\begin{subfigure}{.24\linewidth}
		\centering
		\includegraphics[width=0.99\linewidth]{graphs/pwe-src1_2-m4.eps}
		\caption{src1\textunderscore2 in 4-Model}\label{fig:pwe-sense-mode-src1_2-m4}
	\end{subfigure}
	\begin{subfigure}{.24\linewidth}
		\centering
		\includegraphics[width=0.99\linewidth]{graphs/pwe-src1_2-m5.eps}
		\caption{src1\textunderscore2 in 5-Model}\label{fig:pwe-sense-mode-src1_2-m5}
	\end{subfigure}
\caption{Percentages of blocks with different states, when running \emph{src1\textunderscore2} in 2-Mode, 3-Mode, 4-Mode, and 5-Mode devices.}
\label{fig:pwe-sense-mode-src1_2}
%\vspace{-6pt}
\end{figure*}


\begin{figure*}
\centering
	\begin{subfigure}{.24\linewidth}
		\centering
		\includegraphics[width=0.99\linewidth]{graphs/pwe-wdev_2-m2.eps}
		\caption{wdev\textunderscore2 in 2-Mode}\label{fig:pwe-sense-mode-wdev_2-m2}
	\end{subfigure}
	\begin{subfigure}{.24\linewidth}
		\centering
		\includegraphics[width=0.99\linewidth]{graphs/pwe-wdev_2.eps}
		\caption{wdev\textunderscore2 in 3-Mode}\label{fig:pwe-sense-mode-wdev_2-m3}
	\end{subfigure}
	\begin{subfigure}{.24\linewidth}
		\centering
		\includegraphics[width=0.99\linewidth]{graphs/pwe-wdev_2-m4.eps}
		\caption{wdev\textunderscore2 in 4-Mode}\label{fig:pwe-sense-mode-wdev_2-m4}
	\end{subfigure}
	\begin{subfigure}{.24\linewidth}
		\centering
		\includegraphics[width=0.99\linewidth]{graphs/pwe-wdev_2-m5.eps}
		\caption{wdev\textunderscore2 in 5-Mode}\label{fig:pwe-sense-mode-wdev_2-m5}
	\end{subfigure}
\caption{Percentages of blocks with different states, when running \emph{wdev\textunderscore2} in 2-Mode, 3-Mode, 4-Mode, and 5-Mode devices.}
\label{fig:pwe-sense-mode-wdev_2}
%\vspace{-6pt}
\end{figure*}




\subsubsection{Effectiveness of Our Schemes under Varying Granularities}

In general, the more voltage states, the longer the device lifetime. However, some workloads significantly benefit from increasing the number of modes, while the lifetime gain is negligible in others. Figure \ref{fig:sense-mode-life} shows the lifetime improvement achieved by the 2-Mode, 3-Mode, 4-Mode, and 5-Mode devices in four representative workloads, which are categorized into two groups. (the results for all others are shown in Appendix).


\begin{itemize}[leftmargin=*]
	\item \textbf{Low-beneficial workloads}: As shown in Figure \ref{fig:sense-mode-life-same}, workloads in this category (e.g., prxy\textunderscore0, src1\textunderscore2) benefit less (or negligible) from the increasing number of modes. It is because majority retention times in these workloads are below 10 hours, while the difference among the 2, 3, 4, and 5-Mode devices is the assignment of different voltage modes (2, 4, 5, and 6-state mode, respectively) to blocks whose P/Es are between 30K and 50K (see the last two mapping of the second row in Table \ref{tab:mode-assign-5-sense-mode}).
	\item \textbf{High-beneficial workloads}: For workloads in this group (e.g., web\textunderscore1, wdev\textunderscore2), increasing the number of supporting modes leads to a significant device lifetime improvement (see Figure \ref{fig:sense-mode-life-increase}). These workloads include a large amount of data whose retention times are between 10 hours and 3 days, which can be placed in blocks with finer-granularity state modes such as 6 and 5-state mode in the 4-Mode/5-Mode devices. In contrast, in the 2-Mode/3-Mode devices, such data are accommodated in blocks with 2 and 4-state mode. (compare the third row of Table \ref{tab:mode-assign-5-sense-mode}).
\end{itemize}


The PWE analysis shown in Figure \ref{fig:pwe-sense-mode-src1_2} visualize why a low-beneficial workload (src1\textunderscore2) cannot fully draw the full potential of increasing the number of modes, whereas Figure \ref{fig:pwe-sense-mode-wdev_2} illustrates how a high-beneficial workload (wdev\textunderscore2) experiences a significantly-increased lifespan by supporting more modes. For \emph{src1\textunderscore2}, the cliff at the latter of its lifespan represents that the blocks ``where data whose retention times range from 1 to 10 hours are stored'' change their modes, when their P/E cycles go beyond 30K. Such data can use blocks with 2 (red), 4 (black), 5 (yellow), and 6 (purple) states in the 2-Mode, 3-Mode, 4-Mode, and 5-Mode devices, respectively. Consequently, these small differences do not results in a significant lifetime gain. In contrast, \emph{wdev\textunderscore2} includes a lot of data whose retention times are between 10 hours and 3 days, and such data can be stored in blocks with more states (or higher PWEs) in early P/E cycles (i.e., from 0 to 30K) in the 4-Mode and 5-Mode devices. As a result, one can observe from the 5-Mode device (Figure \ref{fig:pwe-sense-mode-wdev_2-m5}) that the 20\% of total blocks gradually change their modes (i.e., red, black, yellow, and purple areas) throughout the device lifespan, which results in much higher PWEs, compared to the continuous low and unchanged PWE (i.e., ``1'') for the same blocks in the 2-Mode device (see the red area in Figure \ref{fig:pwe-sense-mode-wdev_2-m2}).  





==> eval-setup.tex <==
\section{Experimental Methodology}

\begin{figure}
		\centering
		\includegraphics[width=\columnwidth]{figs/method.eps}
		\caption{The simulation framework consists of (a) simulator, (b) configuration file, (c) trace file, and (d) result file.}
	\label{fig:method}
	%\vspace{-20pt}
\end{figure}

\subsection{Simulation Framework}
We exploited DiskSim simulator \cite{framework2} with the SSD extensions by Microsoft \cite{framework1} to implement our proposed scheme. This widely-used simulation platform is highly-parameterized and modulated, which enables a wide range of customization in flash-based storage. Specifically, it allows one to configure ``storage internals'' such as flash chip count, block count, and page size and ``timings'' such as device access latency and parallelization level. 

On top of this simulator, as illustrated in Figure \ref{fig:method}a, we modeled four functions of our scheme: \emph{retention estimation}, \emph{block allocation}, \emph{garbage collection}, and \emph{data scrubbing}. We newly added the retention estimation and the data scrubbing modules to estimate/classify I/O data based on their inter-update times and move data to safe locations in case of failure of the estimation, respectively. We also modified the block allocation and the garbage collection modules by making the system support multiple active blocks and multiple rounds of blocks, respectively.



\begin{figure}
		\centering
		\includegraphics[width=0.7\columnwidth]{figs/config.eps}
		\caption{Examples of our target system as SCM in a memory hierarchy : (a) SLC cache and (b) SLC buffer.}
	\label{fig:config}
	%\vspace{-20pt}
\end{figure}



\begin{table}
\caption{Baseline storage system configuration.}
\label{tab:base-config}
\small
%\vspace{-10pt}
\begin{tabular}{|c|c|c|  }
\hline 
\multicolumn{3}{|c|}{\textbf{64GB SLC SSD = 8 x 8GB SLC flash chip} \cite{baseline-slc} } \\ 
\hline\hline
Flash configuration	&	Flash timing 	& Other characteristics \\ 
\hline\hline 
8192 blocks / chip	&	Read: 35us		&  Lifespan: 50K P/E cycles \\
128 pages / block	&	Write: 350us 	&  Chip interface: 200MB/s \\
8KB page size		& 	Erase: 1.5ms     &  GC: GREEDY\cite{gc-greedy}+wear-leveling \\ 
\hline
\end{tabular}
%\vspace{-5pt}
%\vspace{-5pt}
\end{table}



\subsection{System Configuration}
Our scheme mainly targets SLC flash-based SCMs. In practice, SLC flash memory is an appropriate element for SCM, as it can provide short response times, compared to slow backend storage. Figure \ref{fig:config} presents two examples of SLC-based SCM in a memory (storage) hierarchy; (a) I/O cache of hard disk drives (data pool) and (b) I/O buffer of high-capacity (MLC/TLC) solid state drives. One point we want to emphasize that such SLC-based SCMs are under high I/O pressure (originally given to the lower-level data storage systems) and our scheme can be quite effective in extending their lifetime.

Hence, we employ an SLC flash-based SSD as our baseline system configuration. Specifically, we assume an 64GB SSD configuration with eight 8GB SLC flash chips, whose characteristics are listed in Table \ref{tab:base-config}. Particularly, we highlight two important points: timing values (35us and 230us for read and write, respectively) and block lifespan (50K P/E cycles), as our purpose is to extend SLC life without sacrificing its response time. Note that all these system configuration information is given to the simulator as a parameter, as shown in Figure \ref{fig:method}b.





\begin{table}
\caption{Assignment of a state mode (2, 4, and 8-state mode) to a block.}
\label{tab:mode-assign-3-base}
\small
%\vspace
\begin{tabular}{|c||c|c|c|c|c|  }
\hline 
\multirow{2}{*}{\textbf{IUT}}		& \multicolumn{5}{|c|}{\textbf{P/E Cycles} } \\ \cline{2-6}
\textbf{(Retention Time)}	&	0$\sim$10K 	&	10$\sim$20K	&	20$\sim$30K	&	30$\sim$40K	&	40$\sim$50K	 \\ 
\hline\hline 
$\sim$1 Hour			&	8	& 	8	&	8	&	8	&	8	\\
\hline 
1 $\sim$10 Hours		&	8	&   	8	&	8	&	4	&	4	\\
\hline 
10 Hours $\sim$ 3 Days	& 	4	&	4	&	4	&	2	&	2	\\
\hline 
3 Days $\sim$ 			& 	2	&	2	&	2	&	2	&	2	\\
\hline
\end{tabular}
%\vspace{-5pt}
%\vspace{-5pt}
\end{table}



\subsection{Evaluated Systems}
We evaluate three different systems. Their flash/SSD configurations are the same as indicated in Table \ref{tab:base-config}, since our proposal is to process more write data (by changing cell modes) in a fixed configuration.

\begin{itemize}[leftmargin=*]
	\item \textbf{Baseline SLC:} Like a default SLC device, it uses 2-state cell mode for all blocks until it reaches its endurance limit (50K P/Es). 
	\item \textbf{Compact SLC with scrubbing (C-SLC + Scrub):} It employs three different cell modes (i.e., 2, 4, and 8-state) and a block can have any of them at each P/E cycle. Each block is also discarded when it reaches the endurance limit (50K P/Es). Write data is stored in a block with one of the three modes, depending on the block age (i.e., experienced P/Es) and the estimated data IUT. (Table \ref{tab:mode-assign-3-base} shows the mapping between the data and the block mode). In case of failure of IUT estimation, the data scrubbing runs and moves valid data to lower-state mode(s). As discussed earlier, the read and write latencies in each round of blocks with 4 or 8-state mode are set to the same as the baseline SLC timings.
	\item \textbf{Compact SLC with perfect prediction (C-SLC + Oracle):} It has the same block allocation and the garbage collection as \textbf{C-SLC+Scrub}, except that we assume the perfect retention prediction. So, this imaginary system does not trigger the data scrubbing and there is no lifetime and bandwidth waste in protecting valid data whose retention times are mis-predicted.
\end{itemize}



\begin{table*}[t]
\centering
\caption{Characteristics of the evaluated workloads.}
%\vspace{-5pt}
\label{tab:workload-cha}
%\small
\begin{tabular}{|l|l|c|c|c|c|c|c|c|}
\hline
	\textbf{Workload} & \textbf{Workload} & \textbf{Write} & \textbf{Write} & \textbf{Read} & \multicolumn{4}{|c|}{\textbf{Ratio of Logical Blocks with Retention Times (\%)}} \\ \cline{6-9}
\textbf{Name}	&   \textbf{Description}   &  \textbf{Ratio (\%)} &  \textbf{Size (KB)} &  \textbf{Size (KB)}     & $\sim$1 Hour & 1 Hour$\sim$10 Hours & 10 Hours$\sim$3 Days & 3 Days$\sim$ \\
\hline\hline
	hm\textunderscore0 & Hardware monitoring		&   64.5   &	  7.4	&   8.3	&	59.8	&	33.7	&	6.4	&	0.1	\\ \hline
        prn\textunderscore0 & Print server			&   89.2   &	  22.8	&   9.7	&      73.3	&	21.9	&	4.8    &	0	\\ \hline
	prn\textunderscore1 & Print server			&   24.7   &	  22.5	&   11.7	&	59.3	&	33.3	&	7.4	&	0	\\ \hline
	proj\textunderscore0 & Project directories		&   87.5   &	  17.8	&   40.9	&      96.7	&      2.7	&	0.5	&	0.1	\\ \hline
	prxy\textunderscore0 & Firewall/web proxy		&   96.9   &	  8.3	&   4.6	&      96.1	&	3.1	&	0.7	&	0.1	\\ \hline
	mds\textunderscore0 & Media server			&   88.1   &	  23.7	&   7.2       &      66.4	&	29.6	&	3.6	&	0.4	\\ \hline
	src1\textunderscore2 & Source control 		&   74.6   &	  19.1	&   32.5	&	87.9	&	7.9	&	4.1	&	0.1	\\ \hline
	src2\textunderscore0 & Source control			&   88.7   &	  8.1 	&   7.1	&	72.5	&	23.3	&	4.0	&	0.2	\\ \hline
	stg\textunderscore0 & Web staging			&   84.8   &	  24.9	&   9.2       &	62.8	&	35.1	&	2.0	&	0.1	\\ \hline    
	usr\textunderscore0 & User home directories	&   59.6   &	  40.9	&   10.3	&	72.9	&	21.9	&	4.8	&	0.4	\\ \hline
	web\textunderscore0 & Web/SQL server		&   70.1   &	  29.9	&   8.6       &	62.7	&	28.7	&	8.4	&	0.2	\\ \hline
	web\textunderscore1 & Web/SQL server		&   45.9   &	  45.9	&   9.2	&	48.3	&	24.0	&	27.7	&	0	\\ \hline		
	wdev\textunderscore0 & Test web server		&   79.9   &	  12.6	&   8.2	&	62.3	&	33.7	&	3.4	&	0.6	\\ \hline
	wdev\textunderscore2 & Test web server		&   99.9   &	  6.1	&   8.1	&	23.7	&	48.8	&	27.5	&	0	\\ \hline
	rsrch\textunderscore0 & Research projects		&   90.7   &	  10.9	&   8.7	&	79.7	&	20.3	&	0	&	0	\\ \hline
\end{tabular}
% \vspace{-10pt}
\end{table*}


\subsection{Evaluated Workloads}
We use MSR Cambridge Traces suite \cite{cambridge} for our evaluations. Even though there are a lot of publicly-available I/O traces, most of them are collections of I/O traces for at most a few hours. However, we need to see real scenarios where blocks are updated for several minutes, hours, days, or beyond weeks, since we leverage a wide range of block retention times in our scheme. To the best of our knowledge, MSR Cambridge traces for one week have the longest history of blocks and we could observe from them that many blocks are updated for up to several days. 

Among 36 traces of MSR Cambridge suite, we selected 15 traces, which are listed in Table \ref{tab:workload-cha}. We exclude the remaining 21 traces, since (1) they are from read-intensive applications or (2) many blocks are shown (logged) only one time in the traces. Specifically, our proposal of extending the storage lifetime is less critical for read intensive applications, though it is still necessary as storage finally comes to the end of its lifetime in the future. Furthermore, traces where many blocks appear once is of no use in our evaluation, as we cannot extract (calculate) retention times or inter-update times from them. In contrast, one can see from Table \ref{tab:workload-cha} that various block retention times (i.e., inter-update times) are exhibited in our evaluated workloads.

Figure \ref{fig:method}c shows an example segment of the I/O trace, where an I/O request has the form of (submission time, type, logical block address, size, other information). It is worthwhile to note that how the retention estimation calculates the retention requirement of the current write data. Let us consider the retention time of the logical block B. When a write (update) request of the block in time T2 is shown for the first time, we store the data in a safe place (i.e., a block with 2-state mode), because we do not know when the block was updated right before and keep its submission time. Later, when the block B is updated again in T51, the retention estimation predicts the retention requirement of block B as the update time difference (i.e., T49) and the data is placed in a block with the appropriate state mode. Note that the access of the block B in T3 is read, which is regardless of the retention time. In the same manner, the estimated retention time of the block A after T4 is T3, based on the difference in the consecutive submission times (i.e., T1 and T4). If the write request of a block appears only one time in the trace (e.g., block C in T50), we treat them as ones with the longest retention time (e.g., a few years).



\subsection{Metrics}
We evaluate our proposed system with the following metrics.

\begin{itemize}[leftmargin=*]
	\item \textbf{Lifetime:} It is inferred as the total data volume (size) written to the storage until it comes to the end of its life. Note that the number of P/E cycles it can endure (i.e., 50K P/Es) remains unchanged in our proposed scheme. Under a fixed endurance limit, the more write data the storage can process, the longer lifetime it has.
	\item \textbf{PWE:} Compared to the baseline SLC where all blocks has 2-state mode (whose PWE is ``1'') in the whole lifetime, C-SLC schemes have a mix of blocks with 2, 4, or 8 state mode (their PWEs are ``1'', ``3'', and ``7'', respectively) and their ratios vary as the P/Es increase and the workload characteristics change. The higher the ratio of blocks with 8 or 4-state mode, the longer the lifetime.
	\item \textbf{GC rate/cost:} The GC rate is the number of GC invocations in a time units, whereas the GC cost represents the average GC execution time (that is taken in performing migrations and erase/dummy write). The higher the GC rate and cost, the larger the waste of storage bandwidth. 
	\item \textbf{Scrubbing rate/cost:} The scrubbing rate indicates how often the data scrubbing is triggered, which is calculated as the ratio of blocks on which the data scrubbing is actually triggered to the total number of block allocated (used). The scrubbing cost is the average number of page migrations (to keep valid data in a safe location). The higher the scrubbing rate and the cost, the larger the waste of storage lifetime and bandwidth.
	\item \textbf{Storage throughput:} It indicates the data volume (size) the storage can process in a unit time.
\end{itemize}

All metric values are generated as a result of the simulation, as shown in Figure \ref{fig:method}d. Except for PWE results, we normalize the results of C-SLC+Scrub and C-SLC+Oracle to that of baseline SLC in the following graphs.

